Pushing the limits of Full-duplex: Design and Real-time Implementation

Recent work has shown the feasibility of single-channel full-duplex wireless physical layer, allowing nodes to send and receive in the same frequency band at the same time. In this report, we first design and implement a real-time 64-subcarrier 10 MHz full-duplex OFDM physical layer, FD-PHY. The proposed FD-PHY not only allows synchronous full-duplex transmissions but also selective asynchronous full-duplex modes. Further, we show that in over-the-air experiments using optimal antenna placement on actual devices, the self-interference can be suppressed upto 80dB, which is 10dB more than prior reported results. Then we propose a full-duplex MAC protocol, FD-MAC, which builds on IEEE 802.11 with three new mechanisms -- shared random backoff, header snooping and virtual backoffs. The new mechanisms allow FD-MAC to discover and exploit full-duplex opportunities in a distributed manner. Our over-the-air tests show over 70% throughput gains from using full-duplex over half-duplex in realistically used cases.

==> basic_two_way.tex <==
\subsection{Shared Random Backoff \label{sec:srb}}



==> eval.tex <==
\section{FD-MAC Evaluation} \label{sec:eval}

\subsection{Two-node Full-duplex}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}\hline
SINR & Througput& Througput \\
& of HD & FD \\ \hline
 
\end{tabular}
\end{table}
%Gaurav's results. Describe the experiment setup, then make sure we use that setup as much as possible to study different aspects - distance, antenna placement, device or not, etc. Be creative.

\subsection{Impact of packet reordering}

%Experiment not possible, so we will analyze. Key is how often nodes
%can use the full-duplex compared to a genie-aided system. There is a
%tradeoff between aggressiveness and collisions etc. See if you can
%compute some formulae, use MATLAB to plot it.
For multiple node topologies, one of the parameters deciding the
throughput is the depth of the buffer at $\mathsf{AP}$,
$\mathsf{Bufdepth}$. Large $\mathsf{Bufdepth}$ is likely to improve
the throughput allowing more and more FD. Since reordering modifies
the head of the buffer, the packet at the head of the buffer will
experience a delay. Without reordering, head of the buffer is always
transmitted and we call that as a delay=0. In
Figure.~\ref{fig:ThptDelay}, we plot the simulated througput
vs. average delay for a network with 5 mobile nodes and an
$\mathsf{AP}$. All nodes always have packets for the $\mathsf{AP}$,
and in radio range of one another. In order to study the parameters
$\mathsf{Bufdepth}$ and $p_{pick}$, only virtual contention is
allowed. The $\mathsf{AP}$ has the same traffic for all nodes and the
order in which packet for different destinations arrive is uniformly
random. The plot shows a key finding that the throughput and average
delay are linearly related. Larger $\mathsf{Bufdepth}$ can help in
improving the throughput at the cost of delay. Also, it is often
possible to obtain the same (throughput, average delay) pair for
smaller $\mathsf{Bufdepth}$ by simply increasing the probabilty of
reordering, $p_{pick}$.

\begin{figure}[ht]
\vspace{-2.9cm}\centering
\includegraphics[scale=0.4]{figs/ThptDelay.pdf}
\label{fig:ThptDelay}
\vspace{-3cm}
\caption{The throughput is normalized, with a maximum value of 2 when
  all packets are in FD and a minimum of 1 when all packets are in
  HD. Number of mobile nodes is 5. Average delay = 0, when no
  reordering ($\mathsf{Bufdepth} = 1$)}
\end{figure}



==> mac.tex <==
\section{MAC Design}

In this section, we describe the main block diagram of our real-time
full-duplex OFDM physical layer and the design space of the MAC
protocol built on the physical layer. We note that full-duplex is a
very young area and hence we expect many innovations in coming years
which will improve upon our current design; some of these ideas are
discussed in Section~\ref{sec:future work}.



\begin{itemize}
\item Introducing the Access Point ($\mathsf{AP}$) + Mobiles based
  system where mobile node can interact in only two kinds of flows
  possible, from $\mathsf{AP}$ to the mobile node or mobile node to
  the $\mathsf{AP}$. Since the $\mathsf{AP}$ is always an interacting
  node, at max only two flows are possible (limited by the number of
  flows that the $\mathsf{AP}$ can handle). Introduce the two possible
  topologies (clique based and linear topology-hidden node topology)
\item Introduce the atomic element of the FD which is the two way
  traffic flow which is possible only if the participating nodes have
  packets are available for each other. Introduce the constraints with
  justification from some experimental results. Describe the possible
  protocols which are handshaking based (RTS/CTS or Data packets with
  additional fields)
\item 3 node system (the clique and the hidden node)

\end{itemize}

\subsection{Access point based topologies}
We study a wireless system which closely resembles the WiFi
network. In this network, fundamentally there are two kinds of nodes:
the Access Point ($\mathsf{AP}$) and the Mobile node. Each
$\mathsf{AP}$ serves a bunch of mobile nodes. The placement of
$\mathsf{AP}$s themselves is frequency planned \textbf{(how much do we
  need to explain here?)}. Since the neighboring $\mathsf{AP}$s use a
different frequency channel, it is sufficient to study a network with
only one $\mathsf{AP}$. The mobile nodes communicate only with the
$\mathsf{AP}$, i.e. the mobile nodes either send a packet to the
$\mathsf{AP}$ or receive a packet from the $\mathsf{AP}$. Every
communication flow has the $\mathsf{AP}$ as a participating node, and
since the $\mathsf{AP}$ can transmit to at most one mobile node and
receive from at most one mobile node at the same time, a maximum of
two simultaneous flows are possible in the network.  Since each mobile
node needs to transmit to or receive from the $\mathsf{AP}$, it is
sufficient to consider only those mobile nodes which have a link to
and from the $\mathsf{AP}$. Since we are considering full-duplex PHY,
it can be assumed that the channels are reciprocal, i.e. if the mobile
node has a link to the $\mathsf{AP}$, the $\mathsf{AP}$ too has a link
to the mobile node. It is instructive to consider a network which has
at most three nodes (one $\mathsf{AP}$ and two mobile nodes)
participating in a communication simultaneously. With one
$\mathsf{AP}$ and two mobile nodes, say $\mathsf{M}_1$ and
$\mathsf{M}_2$, two basic topologies are possible
\begin{figure}[h]
\subfigure[{A clique topology with one $\mathsf{AP}$ and two mobile
    nodes}]{\label{fig:CliqueTop}\resizebox{1.3in}{!}{\input{figs/Clique.pdf_t}}} \hspace{0.2cm}
\subfigure[{A hidden node topology where $\mathsf{M}_1$ and
    $\mathsf{M}_2$ are not in the radio range of each
    other}]{\label{fig:HiddenNodeTop}\resizebox{2.0in}{!}{\input{figs/HiddenNode.pdf_t}}}
\caption{Two possible topologies with a three node network. Any two
  nodes connected via a line implies that they are in the radio range
  of one another}
\label{fig:Topology}
\end{figure}
\begin{enumerate}
\item Clique topology i.e. all nodes can listen to transmission of each other)
\item Hidden node topology i.e. $\mathsf{M}_1$ and $\mathsf{M}_2$ cannot
  listen to transmissions of each other.
\end{enumerate}
The two topologies are depicted in the Fig. \ref{fig:Topology}. Let us
assume that each of the mobile nodes always have a packet to sent to
the $\mathsf{AP}$, i.e. the queues at the mobile nodes are backlogged
and also assume that the $\mathsf{AP}$ has packets to send to all the
mobile nodes at all times. We observe that in a clique topology, only
two possible states are possible which utilize full-duplex and do not
(depict it in a figure) lead to any collisions.  Each of states
depicted in the Fig. is a termed as a two-way flow. Each two-way flow
has only two participating nodes (the $\mathsf{AP}$ and one mobile
node), each of whom send and receive packets from one another. For
ease of understanding, we develop the protocol in several steps by
managing several different states in which full-duplex communication
can happen. At each step, we describe aspects of the protocols which
enable some of the possible states. In Section \ref{subsec:TwoWayFD},
we describe the details of the proposed MAC layer protocol for the
single two-way flow.  In Section \ref{subsec:Clique}, we extend the
MAC protocol design to handle clique topologies and describe how the
protocol allows switching between one two-way flow to another two-way
flow. In the hidden node topology, four different states with
full-duplex are possible where no collisions occur. In Section
\ref{subsec:HiddenNode}, we describe the details of the MAC protocol
which can handle the all states in the hidden node topology with
provision of switching between one state to another.

\begin{figure}[h] \centering
\subfigure[{}]{\label{fig:twoway1}\resizebox{1.0in}{!}{\input{figs/cliqueflows.pdf_t}}} \hspace{0.2cm}
\subfigure[{}]{\label{fig:twoway2}\resizebox{1.0in}{!}{\input{figs/cliqueflows2.pdf_t}}}
\caption{The two possible states in which two flows are possible in a
  clique topology}
\label{fig:twowayflows}
\end{figure}

\begin{figure}[h] \centering
\subfigure[{}]{\label{fig:hiddenNode1}\resizebox{2.0in}{!}{\input{figs/hiddenflows1.pdf_t}}} \hspace{0.2cm}
\subfigure[{}]{\label{fig:hiddenNode2}\resizebox{2.0in}{!}{\input{figs/hiddenflows2.pdf_t}}}
\subfigure[{}]{\label{fig:hiddenNode3}\resizebox{2.0in}{!}{\input{figs/hiddenflows3.pdf_t}}} \hspace{0.2cm}
\subfigure[{}]{\label{fig:hiddenNode3}\resizebox{2.0in}{!}{\input{figs/hiddenflows4.pdf_t}}}
\caption{Four possible states in which two flows are possible in a
  hidden node topology}
\label{fig:hiddenflows}
\end{figure}

\subsection{Two-Way Full-Duplex}
\label{subsec:TwoWayFD}
The smallest number of nodes in a full-duplex communication is two. It
has two flows, one from the $\mathsf{AP}$ to the mobile node
$\mathsf{M}_1$ and vice-versa. Although both $\mathsf{AP}$ and
$\mathsf{M}_1$ are capable of full-duplex communication, traffic
patterns, delay constraints, etc. can result in only one of the nodes
transmitting at a time. In such a scenario, nodes need to capture the
media which similar to that of the half-duplex communication. When the
network is silent, a node captures the media using either a 4-way
handshake (RTS/CTS) \textbf{(add reference)} or a two-way handshake
(basic access) \textbf{(add reference)}. In the FDMAC design, we will
assume that when a node initiates communication with another node
(i.e. starts sending packets to another node), it simply uses the
two-way handshake. Since FDMAC protocol uses two-way handshake, it has
a payload packet and an acknowledgement packet. We define the packet
structure for FDMAC with certian fields in addition to the
conventional fields present in payload and acknowledgement packets
used in half-duplex.

\emph{Packet structure:} Clearly FDMAC with two nodes will have two
differnt states, a half duplex state and a full-duplex state. We
therefore have two kinds of payload packets, a half-duplex packet
denoted by HDPACKET and a full-duplex packet denoted by FDPACKET. Both
the HDPACKET and the FDPACKET consists of training sequence (TRAIN),
packet header (HEADER) with fields for source (S), destination (D) and
packet length (PACLEN), and head of line field (denoted by HOL, it
indicates that the source has another packet at head of the buffer for
the same destination). There is a one bit field, the PACTYPE,
distinguishing the HDPACKET and FDPACKET. In addition to this it has a
PAYLOAD. The structure of the HDPACKET is shown in the
Fig. \ref{fig:hdpacket}.

In order to define the MAC protocol for the two-way full-duplex, we
start from the state where one of the nodes either the $\mathsf{AP}$
or mobile node $\mathsf{M}_1$ is already transmitting packets to the
other. Since the protocol for two-way full-duplex it will be symmetric
for the $\mathsf{AP}$ and $\mathsf{M}_1$, we will assume an initial
state where $\mathsf{AP}$ is in transmitting a packet to the
$\mathsf{M}_1$ and describe the state transition to two-way
full-duplex. In the initial state, i.e. when the only transmitting
node is the $\mathsf{AP}$, it transmits a half-duplex packet
(HDPACKET).

\begin{figure}[h] \centering 
\subfigure[{Design of a half-duplex
    packet/full-duplex packet}]{\label{fig:hdpacket}\resizebox{2.0in}{!}{\input{figs/hdpacket.pdf_t}}}
\subfigure[{Design of the acknowledgment
    packet}]{\label{fig:ackpacket}\resizebox{2.0in}{!}{\input{figs/ackpacket.pdf_t}}}
\caption{Structure of different packets for the FDMAC}
\end{figure}

The initial state of the network is $\mathsf{AP}$ transmitting a
HDPACKET to the mobile node $\mathsf{M}_1$. Suppose that the HOL field
of the current HDPACKET is 1, i.e. the $\mathsf{AP}$ reveals that its
buffer consists of another packet whose destination is
$\mathsf{M}_1$. Also, suppose that while $\mathsf{M}_1$ is receiving
the HDPACKET, a packet arrives in its buffer whose destination is the
$\mathsf{AP}$. Since both the participating nodes have packets for
each other in their respective buffers, there is an opportunity for
setting up a two-way full-duplex flow. From the PHY layer design, we
know that any node engaging into full-duplex communication must have
an estimate of the self-interference channel in order to cancel it
using analog cancellation. The power of self-interference is much
greater than the power of the signal being received, and thus if
$\mathsf{M}_1$ asynchronously decides to transmits its packet to
$\mathsf{AP}$ while the transmission of HDPACKET is going on, it will
collide with the packet it is receiving. A silent slot is therefore
needed to train the self interference channel, which calls for some
form of scheduling using the MAC. In order to set up the two way flow,
$\mathsf{M}_1$ will use the ACK to convey that it has a packet in its
buffer for $\mathsf{AP}$. The conventional acknowledgment packet will
be modified for this purpose. The modified ACK packet consists of a
training sequence (TRAIN) and a header (HEADER). In addition to this,
it has three additional one bit fields: PD (packet for destination)
indicating that sender of the ACK has a packet for the recipient of
the the ACK, PSE (packet for someone else) indicating that the sender
of the ACK has a packet in its buffer for a node other than the
recipient of the ACK and a CTS (clear to send) indicating that the
recipient of the ACK can start transmitting. The structure of the ACK
packet is shown in Fig \ref{fig:ackpacket}. At the end of the
successful HDPACKET reception, $\mathsf{M}_1$ immediately sends an
acknowledgment (ACK) packet to $\mathsf{AP}$ with fields set PD and
CTS set to 1 and PSE set to 0. Since the ACK sent from $\mathsf{M}_1$
has a training sequence TRAIN, $\mathsf{M}_1$ uses it to train the
self-interference channel (\textbf{give the right variable name,
  maybe}), and $\mathsf{AP}$ uses it to train the channel from
$\mathsf{M}_1$ and $\mathsf{AP}$. Now, the $\mathsf{AP}$ needs to
train its own self-interference channel, so at the end of the
reception of ACK from $\mathsf{M}_1$, it immediately captures the
media by transmitting a fake-ACK. The fake-ACK has the same structure
as the ACK packet except that its packet type is set to FA. The
destination of the fake-ACK is $\mathsf{M}_1$ and its PD and CTS
fields are set to 1. The training sequence in fake-ACK is used by
$\mathsf{AP}$ to obtain its estimates of the self interference
channel, while it is used by $\mathsf{M}_1$ to obtain an estimate of
the channel from $\mathsf{AP}$ to $\mathsf{M}_1$. At the end of
transmission of the fake-ACK, both $\mathsf{AP}$ and $\mathsf{M}_1$
immediately start transmitting in full-duplex mode their respective
full-duplex packet. The full-duplex packets has the same structure as
the half-duplex packet except that its packet type field is set to
FD. The packet lengths of the two FDPACKETs can be different. If both
the FDPACKETs have their HOL fields are set to 1, their is an
opportunity for another round of full-duplex exchange. Once the
longer of the two packets finishes transmitting, the node which
initiated the full-duplex two-way flow, in this case $\mathsf{M}_1$,
replies back with an ACK. Following the transmission of ACK from
$\mathsf{M}_1$, the $\mathsf{AP}$ will reply with an ACK. If the HOL
fields of both the FDPACKETs were set to 1, the ACK to and from
$\mathsf{M}_1$ will have fields PD and CTS set to 1, and then another
round of full-duplex ensues. The set-up of a full-duplex flow from an
initial state of a half-duplex flow is shown in the
Fig. \ref{fig:twowaysetup}.

\begin{figure}[h]
\centering
\label{fig:hdpacket}\resizebox{3.5in}{!}{\input{figs/twowaysetup.pdf_t}}
\caption{Setting up of the two-way full duplex flow from an initial
  state of half-duplex}
\label{fig:twowaysetup}
\end{figure}

If any of the two FDPACKETs had the HOL fields were set to 0, the next
state will be a half-duplex like transmission which will start with
the two-way handshake (i.e. transmission of an HDPACKET from the
source (either $\mathsf{AP}$ or $\mathsf{M}_1$ followed by the ACK by
the recipient). If neither of the nodes have no packets to send to
each other, the network simply becomes silent after the exchange of
ACKs with HOL fields of both the FDPACKETs set to 0, and PD field of
both the ACKs also set to 0.

In this section, we have discussed the state transition from a
half-duplex flow to a full-duplex two-way flow and vice
versa. However, this protocol supports networks with only two
nodes. Suppose that there were other mobile nodes present in this
network, it would not allow them to communicate with the $\mathsf{AP}$
as long as $\mathsf{AP}$ and $\mathsf{M}_1$ have packets for another
(the channel will be permanently occupied by FDPACKETs and ACKs), thus
allowing no room for contention of the channel. In the next section we
present modification to the MAC protocol to accomodate more than one
mobile node if the nodes form a clique topology. We explain the
protocol with describe

\subsection{Clique Topology}
\label{subsec:Clique}
We first discuss a clique topology with one $\mathsf{AP}$ and two
mobile nodes $\mathsf{M}_1$ and $\mathsf{M}_2$. As described in
section \ref{subsec:TwoWayFD}, half-duplex transmission can be
achieved via two way handshake. A two-way full-duplex can be set up by
the protocol described in section \ref{subsec:TwoWayFD}. In this
section add elements to the protocol to enable a state transition from
one two-way full-duplex flow, say between $\mathsf{AP}$ and
$\mathsf{M}_1$ to another two-way full-duplex flow, say between
$\mathsf{AP}$ and $\mathsf{M}_2$.
\begin{figure}[h]
\resizebox{2.5in}{!}{\input{figs/cliquestates.pdf_t}}
\caption{State transition from one two-way full-duplex flow (between
  $\mathsf{AP}$ and $\mathsf{M}_1$) to another two-way full-duplex
  flow (between $\mathsf{AP}$ and $\mathsf{M}_2$) in a clique
  topology. A similar state transition diagram can be drawn}
\label{fig:cliquestates}
\end{figure}
In the protocol for two-way full-duplex flow, there is no opportunity
for the nodes not interacting in the full-duplex flow to capture the
media. Moreover, the $\mathsf{AP}$ has a buffer in which packets
intended for different mobile nodes are placed in the order they
arrive. 

\emph{some important text}

The MAC protocol allows contention via two forms of random access 1)
Physical contention and 2) Virtual contention. Physical contention is
intended for mobile node $\mathsf{M}_2$ to contend for the media while
two-way full-duplex flow between $\mathsf{AP}$ and $\mathsf{M}_1$ is
going on. At the end of every round of full-duplex FDPACKET exchange,
ACKs are exchanged between $\mathsf{AP}$ and $\mathsf{M}_1$. Since the
topology is clique, $\mathsf{M}_2$ is able to listen to the ACKs
transmitted by the $\mathsf{AP}$ and $\mathsf{M}_1$. Thus it clearly
knows the start and end of both the ACKs. At the end of ACKs, the
FDPACKETs start again, if both $\mathsf{AP}$ and $\mathsf{M}_1$ have
packets for each other. Instead of allowing the $\mathsf{AP}$ and
$\mathsf{M}_1$ to immediately capture the media, the $\mathsf{AP}$ and
$\mathsf{M}_1$ back-off by a predetermined amount of time. Both
$\mathsf{AP}$ and $\mathsf{M}_1$ generate a random number between 0
and their respective maximum contention window
$\mathsf{CW}_\mathrm{max}$ and then share it using their ACKs. The ACK
has a field for random back-off denoted by RAB. The $\mathsf{AP}$ and
$\mathsf{M}_1$ pick the maximum of the two RABs and remain silent for
that long before transmitting their FDPACKETs. The node $\mathsf{M}_2$
can use this period to contend for the media by generating its own
random back-off and then capturing the media if possible. If
$\mathsf{M}_2$ captures the media during this contention period, then
$\mathsf{AP}$ and $\mathsf{M}_1$ do not transmit anymore and the state
transits into a one-way half-duplex flow. If $\mathsf{AP}$ has packets
for $\mathsf{M}_2$ in its buffer, then via the two-way full-duplex
flow setup as described in section \ref{subsec:TwoWayFD}, the state
can easily transit to the two-way full-duplex flow between
$\mathsf{AP}$ and $\mathsf{M}_2$. Under high traffic, i.e. when all
mobile nodes have packets for $\mathsf{AP}$ and vice versa, remaining
in a single two-way full-duplex once it has been set up gives high
throughput. Every state transition from one two-way full-duplex flow
to another two-way full-duplex flow has an intermediate half-duplex
flow. In order to ensure improvement in throughput, the protocol
ensures that the nodes exchanging packets in full-duplex will have a
zero back-off time, the first time they exchange FDPACKETs after
exchanging ACKs. The shared random backoff is used only the second
FDPACKET exchange onwards.  \\

\emph{talk a little bit about why shared back-off and not arbitrary
  back-off} \\

Virtual contention is needed for allowing the packets in the buffer of
the $\mathsf{AP}$ to contend for channel. Packets arrive in the buffer
in an arbitrary order. In 802.11, the packets are transmitted in a
first-in-first-out manner. Since the packets arrive in an arbitrary
order, there is no guarantee that the $\mathsf{AP}$ will have
consecutive packets for the same destination to engage in a
full-duplex communication for a long time. In order to improve the
likelihood of having packets for the same destination, the depth of
the buffer from which the packets are being picked must be
increased. We denote the depth of the buffer by BUFDEPTH. Larger
BUFDEPTH implies more likelihood of remaining in a two-way
full-duplex. At the same time larger BUFDEPTH may lead to large delays
for packets which arrive early but do not belong to the destination
with which $\mathsf{AP}$ is engaged in full-duplex communication. Thus
to allow fairness between choice of destinations, the protocol allows
a contention between the current destination (as long as there is a
packet meant for it with the BUFDEPTH of $\mathsf{AP}$'s buffer) and
the destination of the packet which is on the head of the buffer. The
protocol picks the current destination with a probability of 0.5 and
the head of the buffer packet with probability 0.5. If the head of the
buffer packet is not meant for the current destination, the
$\mathsf{AP}$ modifies it's ACK field PSE to 1 and PD to zero
indicating that it has a packet for someone else. It then contends for
the channel via two-way handshake and engages into half-duplex
communication if its contention was successful. There is a natural
tradeoff between the depth of the buffer and the expected delay of the
packet. \\

\emph{some analysis needed here to find the delay vs throughput plots} \\

Although the protocol has been depicted with only mobile nodes, it
applies to a clique topology with any number of nodes since all the
elements of the protocol are independent of the number of nodes. The
choice of BUFDEPTH and the probability for choosing the head of the
buffer as the packet to transmit are parameters which need to be
decided depending on the size of the network.


\subsection{Hidden Node Topology}
\label{subsec:HiddenNode}
Topologies in network are not limited to cliques. Often nodes are
hidden with respect to one another. In this section we highlight the
elements of protocol which enable full-duplex communication in hidden
node topologies. In Fig. \ref{fig:hiddenflows}, 4 different states
with two flows in a hidden node topology was shown. All the four
states have $\mathsf{AP}$ interacting with two flows while the mobile
nodes may have one or two flows depending on the state. In this
section, we will add elements to the MAC protocol which will enable
setting up some of the states and state transitions among the states
in the hidden node topology. Note that the nodes are not aware of the
topology and the topologies may change over time. We will first
describe the elements of the protocol needed to enable certain states
and then analyze the state transition.

\emph{Protocol:} Consider the state when $\mathsf{AP}$ is transmitting
a packet to $\mathsf{M}_1$. And suppose that mobile node
$\mathsf{M}_2$ has a packet for the $\mathsf{AP}$ in its buffer. There
are two kinds of packet $\mathsf{AP}$ can transmit based on which the
action of $\mathsf{M}_2$ will be different. \\

\emph{important to change the two way fd protocol to have AP be the
  second one to send the ACK} \\


 \noindent 1) $\mathsf{AP}$ is transmitting an FDPACKET to
 $\mathsf{M}_1$ and $\mathsf{M}_2$. The exchange of FDPACKETs is
 followed by the ACKs and the ACK from $\mathsf{AP}$ comes right
 before the contention period. $\mathsf{M}_2$ waits for the ACK from
 $\mathsf{AP}$ to finish, and then contends for media access and if it
 succeeds it transmits an HDPACKET to $\mathsf{AP}$ thus initiating
 its connection with the $\mathsf{AP}$.

\noindent 2) $\mathsf{AP}$ is transmitting an HDPACKET to
$\mathsf{M}_1$. If the HOL field of the HDPACKET is 0, it implies that
$\mathsf{AP}$ the destination of the next packet is not $\mathsf{M}_1$
(\textbf{unless} $\mathsf{M}_1$ \textbf{requests to go into
  full-duplex}). $\mathsf{M}_2$ waits for one ACK period at the end of
the HDPACKET and then contends for the media. However, if the AP has
the HOL field of the HDPACKET set to 1, and if the ACK from
$\mathsf{M}_1$ is not heard at $\mathsf{M}_2$, then $\mathsf{M}_2$ has
an opportunity to transmit to AP while AP transmits to $\mathsf{M}_1$
(if the ACK is not heard, then it is very likely that $\mathsf{M}_1$
and $\mathsf{M}_2$ are not in radio range of one another, since ACK
error probability is very small), thus enabling two flows at the same
time. Since AP has to both send and receive packets, the PHY layer
constrains it to train its self interference channel before receiving
any other packets. The node $\mathsf{M}_2$ therefore waits for the
$\mathsf{AP}$ to transmit its HDPACKET. It then decodes the header of
the packet to find the PACLEN and then sends an HDPACKET with the size
of the payload adjusted such that it finishes transmission no later
than the transmission of the HDPACKET of $\mathsf{AP}$ \textbf{(show
  figure)}. First $\mathsf{M}_1$ transmits ACK meant for $\mathsf{AP}$
and then $\mathsf{AP}$ transmits an ACK meant for
$\mathsf{M}_2$. Following the ACKs there is a contention period and
$\mathsf{M}_2$ will allow $\mathsf{AP}$ to capture the media if the
ACK from $\mathsf{M}_1$ is not heard at $\mathsf{M}_2$ and
$\mathsf{AP}$ sets it HOL to be 1. (\emph{there are several states
  that can occur and we can discuss the state transitions separately})

\emph{another protocol where the HDPACKET itself can be broken into a
  header, a contention slot and } \\

\emph{we will use shorthand notation for the states, right now i am
  introducing it here but will move it in the beginning of this section
  later} \\ if a packet is being transmitted from node $A$ to node $B$
then we denote it by $A \rightarrow B$. Two-way FD is denoted by $A
\rightleftarrows B$. When $A$ is transmitting to $B$ and $B$ is
transmitting to $C$ simultaneously, it is denoted by the $A
\rightarrow B \rightarrow C$. \\


\emph{State transitions:} The state transitions in the hidden node
topology can be classified into six different categories and we
describe how the protocol supports each one:

\noindent 1) One half duplex transmission to another half-duplex
transmission. This can be further sub-classified into two categories:
\begin{itemize}
\item[a] The state transition $\mathsf{AP} \rightarrow \mathsf{M}_1$
  to $\mathsf{AP} \rightarrow \mathsf{M}_2$ happens simply because the
  head of line packet in the buffer is intended for $\mathsf{M}_2$
\item[b] Rest of the half-duplex to half-duplex transitions happen via
  physical contention of the media by contending half-duplex flows.
\end{itemize}

\noindent 2) State transition from $\mathsf{AP} \rightarrow
\mathsf{M}_1$ to $\mathsf{AP} \rightleftarrows \mathsf{M}_1$ in
presence of the hidden node $\mathsf{M}_2$. The fake-ACK from
$\mathsf{AP}$ captures the immediately one ACK period after the finish
of the HDPACKET from $\mathsf{AP}$. The fake-ACK from $\mathsf{AP}$ is
heard by $\mathsf{M}_2$ which is indicative of a two-way full-duplex
transmission and therefore $\mathsf{M}_2$ will not transmit thus
avoiding collision of packets at $\mathsf{AP}$.\\

\noindent 3) State transition from $\mathsf{AP} \rightarrow
\mathsf{M}_1$ to $\mathsf{M}_2 \rightarrow \mathsf{AP} \rightarrow
\mathsf{M}_1$. The $\mathsf{AP}$ has its HOL field set to 1 in the
HDPACKET. At the end of the current HDPACKET, ACK is transmitted from
$\mathsf{M}_1$ which is not heard by $\mathsf{M}_2$. It does not
contend for the channel in order to enable a full-duplex flow. Once
the HEADER of the HDPACKET from $\mathsf{AP}$ to $\mathsf{M}_1$ is
decoded, $\mathsf{M}_2$ uses it modify its PACLEN suitably
($\mathsf{M}_2 \rightarrow \mathsf{AP}$ should end no later than
$\mathsf{AP} \rightarrow \mathsf{M}_1$). $\mathsf{M}_1$ then initiates
transmission of its HDPACKET thus setting up $\mathsf{M}_2 \rightarrow
\mathsf{AP} \rightarrow \mathsf{M}_1$.\\

\noindent 4) State transition from $\mathsf{M}_2 \rightarrow \mathsf{AP}
\rightarrow \mathsf{M}_1$ to $\mathsf{AP} \rightleftarrows
\mathsf{M}_1$. Suppose the HOL field of the HDPACKET from
$\mathsf{AP}$ was set to 1, it implies that $\mathsf{AP}$ has a packet
at the head of the buffer for $\mathsf{M}_1$. At the end of the
HDPACKET from $\mathsf{AP}$, ACK from $\mathsf{M}_1$ is received at
$\mathsf{AP}$ with the PD field set to 1. $\mathsf{AP}$ then transmits
an ACK to $\mathsf{M}_1$ setting its PD field to 0, PSE to 1 and CTS
to 0. Since HOL of HDPACKET from $\mathsf{AP}$ was set to 1, and PD of
ACK from $\mathsf{M}_1$ was also 1, FDPACKETs can start immediately
after the end of ACK from $\mathsf{AP}$, while $\mathsf{M}_2$ will
remain silent as the CTS it has received was 0.\\

%for Mobile node $\mathsf{M}_2$ is in the radio range of $\mathsf{AP}$
%and listens to the transmission of $\mathsf{AP}$. At the end of the
%HDPACKET, $\mathsf{M}_1$ sends an ACK. If the ACK is not heard by
%$\mathsf{M}_2$, it assumes that $\mathsf{M}_1$ is not in the radio
%range of $\mathsf{M}_2$.

\noindent 5) State transition from $\mathsf{M}_2 \rightarrow
\mathsf{AP} \rightarrow \mathsf{M}_1$ to $\mathsf{M}_2
\rightleftarrows \mathsf{AP}$. Suppose the HDPACKET of $\mathsf{M}_2$
has the HOL field set to 1, and suppose via virtual contention of
packets in the buffer $\mathsf{AP}$ has decided makes the packet for
$\mathsf{M}_2$, its head of line packet. At the end of the full-duplex
$\mathsf{M}_2 \rightarrow \mathsf{AP} \rightarrow \mathsf{M}_1$,
$\mathsf{AP}$ receives an ACK from $\mathsf{M}_1$ and then sends an
ACK to $\mathsf{M}_2$ setting PD to 1, PSE to 0 and CTS 1, thus
requesting $\mathsf{M}_2$ to engage in two-way full-duplex flow. The
FDPACKETs can be exchanged immediately after the end of the ACK from
$\mathsf{AP}$. \\


\noindent 6) State transition from any state which has two flows to
single flow can happen when a mobile node not participating in the
full-duplex flow captures the media in the contention period available
every full-duplex flow. This state transition can also happen when the
$\mathsf{AP}$, via virtual contention, decides to send a packet to a
mobile node not involved in the full-duplex flow. \\

\emph{include the figures of all the state transitions} \\

\emph{discussion about how the protocols will work if there is a
  mixture of hidden node and clique topology... this discussion is not
  very complex} \\

\emph{Note that the hidden node problem is not being solved}




\subsection{MAC Protocol Design Space}

What is the fundamental limitations in MAC. Channels are unknown, so
AGC does not know where to settle. So requires measurement to settle
AGC.


